Stochastic Digital Twin for Copy Detection Patterns

Copy detection patterns (CDP) present an efficient technique for product protection against counterfeiting. However, the complexity of studying CDP production variability often results in time-consuming and costly procedures, limiting CDP scalability. Recent advancements in computer modelling, notably the concept of a "digital twin" for printing-imaging channels, allow for enhanced scalability and the optimization of authentication systems. Yet, the development of an accurate digital twin is far from trivial. This paper extends previous research which modelled a printing-imaging channel using a machine learning-based digital twin for CDP. This model, built upon an information-theoretic framework known as "Turbo", demonstrated superior performance over traditional generative models such as CycleGAN and pix2pix. However, the emerging field of Denoising Diffusion Probabilistic Models (DDPM) presents a potential advancement in generative models due to its ability to stochastically model the inherent randomness of the printing-imaging process, and its impressive performance in image-to-image translation tasks. This study aims at comparing the capabilities of the Turbo framework and DDPM on the same CDP datasets, with the goal of establishing the real-world benefits of DDPM models for digital twin applications in CDP security. Furthermore, the paper seeks to evaluate the generative potential of the studied models in the context of mobile phone data acquisition. Despite the increased complexity of DDPM methods when compared to traditional approaches, our study highlights their advantages and explores their potential for future applications.

==> mobile_results.tex <==
\input{tables/final_iphone_v2}

\input{tables/final_samsung_v2}


\subsection{Mobile phone data results}
\label{sec:mobile phone data}


The results obtained for the data enrolled by the iPhone and Samsung mobile phones are given in Tables \ref{table:final_iphone} and \ref{table:final_samsung} respectively. In both tables the first row \textit{W/O processing} shows simple metrics calculation on the data without any processing, i.e., worst case scenario. 

It should be noted that the results obtained for the FID metrics, i.e., $\xtot$ and $\ttox$, are quite unstable and differ a lot between the models. The other metrics demonstrate more coherent results. For the \Palette model due to its stochastisity for each input the final output was obtained via averaging (mean) of the predictions of 21 realizations. 

For both mobile phones the results of MSE and SSIM metrics are almost identical for \Palette and \TRBpairdUNET while the last one outperforms Pallet on the Hamming distance. The results obtained for the other models are worse but not very significantly. On average the worst results correspond to CycleGAN.


 




==> scanner_results.tex <==
\section{Scanner data results}
\label{sec:scanner data}

\input{tables/final_scanner_2021_v2}

The results obtained on the scanner data are given in Table \ref{table:final_scanner_2021}. The first row \textit{W/O processing} shows simple metrics calculation on the data without any processing, i.e., worst case scenario. It is interesting to note that both FID are extremely bad while the results for the other metrics is more sensible. For example, the Hamming distance between the digital template and printed code binarized via {\color{red} ????} is a little bit worse that the CUT estimation and only about two times worse than the pix2pix and CycleGAN. {\color{red} to continue ...}


==> tables/final_iphone.tex <==
\begin{table*}
	\renewcommand{\arraystretch}{\AS}
	\centering
	\caption{
		Models performance on the normalized iPhone data}
	\label{table:final_iphone}
	\begin{tabular}{lSS[round-precision=3]SS[round-precision=3]S[round-precision=3]}
		\toprule
		\ResultsHeader \\

  
        \midrule
        
		\IT W/O processing    & \IT 289.678181 & \IT 0.30022239 & \IT 289.6819465 & \IT 0.253814172 & \IT 0.248902909 \\
		\pixp                 & 11.81894319    & 0.2317964      & 11.6395675      & 0.005319244     & 0.9100902       \\
		\CyG                  & 20.6922318     & 0.2675648      & 12.5880169      & 0.013846471     & 0.782084        \\
		\TRBpairdOne          &    6.5583569 & 0.239011       &   10.198015   & 0.004931163     & 0.9144482       \\
		\TRBpairdUNET         & 35.34934648    & \B 0.209730192 & 12.22193446     &  0.0043456    & \B 0.924969395  \\
        \Palette & \B 4.637709366 & 0.21642876334561603 & \B 8.995346424 & \B 0.004251883 & 0.91525 \\

		\bottomrule
	\end{tabular}
\end{table*}


==> tables/final_samsung.tex <==
\begin{table*}
	\renewcommand{\arraystretch}{\AS}
	\centering
	\caption{
		Models performance on the normalized Samsung data}
	\label{table:final_samsung}
	\begin{tabular}{lSS[round-precision=3]SS[round-precision=3]S[round-precision=3]}
		\toprule
		\ResultsHeader \\
		\midrule
  
		\IT W/O processing    & \IT 381.4423888 & \IT 0.3138391 & \IT 381.4412639 & \IT 0.2779328 & \IT 0.1934390 \\
		\pixp                 & 8.52850107      & 0.2412255     & 20.1809162      & 0.003993872   & 0.9080927     \\
		\CyG                  & 8.8477716       & 0.2828304     & 22.8469538      & 0.015321453   & 0.6941577     \\
		\TRBpairdOne          & 7.0146882    & 0.2473030     & 17.345934    & 0.0036845     & 0.9135600     \\
		\TRBpairdUNET         & 54.8011773      & \B 0.2106384  & 28.8833209      & \B 0.0032350  & \B  0.9217238 \\
        \Palette & \B 4.4597610 & 0.21911774258314437 & \B 10.7206036 & 0.0040886 & 0.9053354 \\
        
		\bottomrule
	\end{tabular}
\end{table*}


==> tables/final_scanner_2021.tex <==
{
\renewcommand{\arraystretch}{\AS}

\begin{table*}
	\centering
	\caption{
		Models performance on the Scanner data}
	\label{table:final_scanner_2021}
	\begin{tabular}{lSSSS[round-precision=3]S}
		\toprule
		\ResultsHeader \\
		\midrule

		\IT W/O processing    & \IT 304.126018 & \IT 0.237533 & \IT 304.014282 & \IT 0.180703 & \IT 0.479932 \\
		\pixp                 & 3.3739524      & 0.1111944    & 8.5724194      & 0.0451773    & 0.7577989    \\
		\CyG                  & 3.865300       & 0.154900     & \B 4.450700    & 0.048995     & 0.731500     \\
		\TRBpairdOne          & 3.164000    & \B 0.085500  & 6.604900       & 0.040000     & \B 0.778700  \\
		\TRBpairdUNET         & 6.211300       & 0.100200     & 28.109900      & \B 0.036312  & 0.777500     \\
        \Palette & \B 2.923636 & \yb{?} & \yb{?} & \yb{?} & \yb{?}  \\

		\bottomrule
	\end{tabular}
\end{table*}

}

==> variance.tex <==
\subsection{\Palette model stochasticity}

\input{figures/stochasticity}

The DDPM model demonstrates stochastic behaviour, which refers to the generation of multiple outputs for a given input. This characteristic can be advantageous for estimating the non-deterministic properties of the printing-imaging channel. In \autoref{fig:stochasticity}, we illustrate the diverse stochastic estimations $\xe$ and $\te$ when passing through the \Palette model the same digital $\t$ or printed $\x$ template as input.




\subsection{Reliable patterns}

\input{figures/bit_flipping}
\input{figures/std_per_pattern}


Another important application of stochastic generation is determining reliable patterns \cite{Tutt2022wifs}, i.e.\ local blocks that could be printed without bit-flipping due to the dot-gain. As shown in \autoref{fig:bit_flipping_iphone} the probability of flipping is close between real and synthetic samples. Pearson correlation between the probability of bit-flipping computed from $\x$ and $\xe$ for iPhone is $0.9991$. 


\subsection{Uncertainty estimation}

\input{figures/2d_std}

By utilizing the stochastic nature of the DDPM model it is possible to generate uncertainty estimation maps for a given template. By taking std of generated realizations $\{\xe_i^{(k)}\}_{k=1}^K$ for a selected $\t_i$ we could estimate the dot gain of a printer and regions with more randomness. Or, in the reverse path, we could produce where could occur bit-flipping when estimating $\ze$ from $x$. In \autoref{fig:2d_std} \yb{are shown}

\subsection{Pattern stochasticity}


Furthermore, aggregating by pattern type could be performed. In \autoref{fig:std_per_pattern_iphone} \yb{are shown}. It is clearly visible that some patterns are more stable than others. 




